Variational Sequential Labelers for Semi-Supervised Learning

We introduce a family of multitask variational methods for semi-supervised sequence labeling. Our model family consists of a latent-variable generative model and a discriminative labeler. The generative models use latent variables to define the conditional probability of a word given its context, drawing inspiration from word prediction objectives commonly used in learning word embeddings. The labeler helps inject discriminative information into the latent space. We explore several latent variable configurations, including ones with hierarchical structure, which enables the model to account for both label-specific and word-specific information. Our models consistently outperform standard sequential baselines on 8 sequence labeling datasets, and improve further with unlabeled data.

==> diagram.tex <==

\begin{tikzpicture}
  [node distance=1.5em,
  start chain=going above,
  scale=0.5,
  every node/.style={scale=0.5}]
	 \node[bignode, circlechain] (l01) {$z$};
	 \draw[->,thin] (l01.south) |-+(0,-3em)-> (l01);
	 \node[bignode, below=1.5em of l01] (in1) {$x$};
	 \node[bignode, above=1.0em of l01] (out1) {$x$};
	 \draw[->,thin] (l01.north)-> (out1);
     % model diagram
	 \node[punktchain, right= 2.5em of l01] (l11) {BiGRU};
	 \node[punktchain2, join, above=1.0em of l11] (l12) {Latent Structure};
	 \draw[->,thin] (l11.south) |-+(0,-3em)-> (l11);
	 \node[bignode, below=1.5em of l11] (in1) {$x_t$};
	 \node[bignode, above=1.0em of l12] (out1) {$x_t$};
	 \draw[->,thin] (l12.north)-> (out1);
     \draw[->,thin] (l11.west)|-+(-1.5em,0)-> (l11.west);
      \draw[->,thin] (l11.east) -> (l11.east)|-+(1.5em,0) ;
    % first one
	 \node[punktchain, right= 2.5em of l11] (l21) {BiGRU};
	 \node[bignode, circlechain, join] (c22) {$z_t$};
	 \draw[->,thin] (l21.south) |-+(0,-3em)-> (l21);
	 \draw[->,thin] (c22.north) |-+(0,3em) (c22);
	 \node[bignode, below=1.5em of l21] (in2) {$x_t$};
	 \node[bignode, above=1.5em of c22] (out2) {$x_t$};
	 \node[bignode, right=1.0em of out2] (out23) {$l_t$};
	 \draw[->,thin] (c22.400) -> (out23.south);
     \draw[->,thin] (l21.west)|-+(-1.5em,0)-> (l21.west);
      \draw[->,thin] (l21.east) -> (l21.east)|-+(1.5em,0) ;
    % second one
	 \node[punktchain, right= 2.5em of l21] (l31) {BiGRU};
	 \node[bignode, circlechain, join] (c32) {$z_t$};
	 \node[bignode, circlechain, right= 0.5em of c32] (c33) {$y_t$};
     \draw[->,thin] (l31.north) -> (c32.south);
     \draw[->,thin] ($(l31.north)+(0.3em,0)$) -> (c33.250);
	 \node[bignode, below=1.5em of l31] (in3) {$x_t$};
	 \node[bignode, above=1.5em of c32] (out3) {$x_t$};
	 \node[bignode, right=1.1em of out3] (out33) {$l_t$};
     \draw[->,thin] (c32.north) -> (out3.south);
     \draw[->,thin] (c33.north) -> (out33.south);
     \draw[->,thin] (c33.110) -> ($(out3.south)+(0.3em,0)$);
     \draw[->,thin] (in3.north) -> (l31.south);
     \draw[->,thin] (l31.west)|-+(-1.5em,0)-> (l31.west);
      \draw[->,thin] (l31.east) -> (l31.east)|-+(1.5em,0);
  \end{tikzpicture}
  
 

==> diagram2.tex <==

\begin{tikzpicture}
  [node distance=1.5em,
  start chain=going above,
  scale=0.5,
  every node/.style={scale=0.5}]
    % first one
	 \node[punktchain] (l11) {BiGRU};
	 \node[bignode, circlechain, join] (c12) {$z_t$};
	 \node[bignode, circlechain, right= 0.5em of c12] (c13) {$y_t$};
     \draw[->,thin] (l11.north) -> (c12.south);
     \draw[->,thin] ($(l11.north)+(0.3em,0)$) -> (c13.250);
	 \node[bignode, below=1.5em of l11] (in1) {$x_t$};
	 \node[bignode, above=1.5em of c12] (out1) {$x_t$};
	 \node[bignode, right=1.1em of out1] (out11) {$l_t$};
     \draw[->,thin] (c12.north) -> (out1.south);
     \draw[->,thin] (c13.north) -> (out11.south);
     \draw[->,thin] (c13.west) -> (c12.east);
     \draw[->,thin] (in1.north) -> (l11.south);
     \draw[->,thin] (l11.west)|-+(-1.5em,0)-> (l11.west);
      \draw[->,thin] (l11.east) -> (l11.east)|-+(1.5em,0) ;
    % second one
	 \node[punktchain, right= 2.5em of l11] (l21) {BiGRU};
	 \node[bignode, circlechain, join] (c22) {$z_t$};
	 \node[bignode, circlechain, right= 0.5em of c22] (c23) {$g_t$};
     \draw[->,thin] (l21.north) -> (c22.south);
     \draw[->,thin] ($(l21.north)+(0.3em,0)$) -> (c23.250);
	 \node[bignode, below=1.5em of l21] (in2) {$x_t$};
	 \node[bignode, above=1.5em of c22] (out2) {$x_t$};
     \draw[->,thin] (c22.north) -> (out2.south);
     \draw[->,thin] (c23.west) -> (c22.east);
     \draw[->,thin] (in2.north) -> (l21.south);
     \draw[->,thin] (l21.west)|-+(-1.5em,0)-> (l21.west);
      \draw[->,thin] (l21.east) -> (l21.east)|-+(1.5em,0) ;
    % third one
	 \node[punktchain, right= 2.5em of l21] (l31) {BiGRU};
	 \node[bignode, circlechain, join] (c32) {$z_t$};
	 \node[bignode, circlechain, right= 0.5em of c32] (c34) {$u_t$};
	 \node[bignode, circlechain, right= 0.5em of c34] (c33) {$y_t$};
     \draw[->,thin] (l31.north) -> (c32.south);
     \draw[->,thin] ($(l31.north)+(3.0em,0)$) -> (c33.250);
     \draw[->,thin] ($(l31.north)+(1.0em,0)$) -> (c34.240);
	 \node[bignode, below=1.5em of l31] (in3) {$x_t$};
	 \node[bignode, above=1.5em of c32] (out3) {$x_t$};
	 \node[bignode, above=1.5em of c33] (out33) {$l_t$};
     \draw[->,thin] (c32.north) -> (out3.south);
     \draw[->,thin] (c33.north) -> (out33.south);
     \draw[->,thin] (c33.west) -> (c34.east);
     \draw[->,thin] (c34.west) -> (c32.east);
     \draw[->,thin] (in3.north) -> (l31.south);
     \draw[->,thin] (l31.west)|-+(-1.5em,0)-> (l31.west);
      \draw[->,thin] (l31.east) -> (l31.east)|-+(1.5em,0) ;
    % forth one
	 \node[punktchain, right= 2.5em of l31] (l41) {BiGRU};
	 \node[bignode, circlechain, join] (c42) {$z_t$};
	 \node[bignode, circlechain, right= 0.5em of c42] (c44) {$u_t$};
	 \node[bignode, circlechain, right= 0.5em of c44] (c43) {$g_t$};
     \draw[->,thin] (l41.north) -> (c42.south);
     \draw[->,thin] ($(l41.north)+(3.0em,0)$) -> (c43.250);
     \draw[->,thin] ($(l41.north)+(1.0em,0)$) -> (c44.240);
	 \node[bignode, below=1.5em of l41] (in4) {$x_t$};
	 \node[bignode, above=1.5em of c42] (out4) {$x_t$};
     \draw[->,thin] (c42.north) -> (out4.south);
     \draw[->,thin] (c43.west) -> (c44.east);
     \draw[->,thin] (c44.west) -> (c42.east);
     \draw[->,thin] (in4.north) -> (l41.south);
     \draw[->,thin] (l41.west)|-+(-1.5em,0)-> (l41.west);
      \draw[->,thin] (l41.east) -> (l41.east)|-+(1.5em,0) ;
  \end{tikzpicture}


==> graphical_plots/3gaussian.tex <==
\begin{tikzpicture}
  [node distance=1.5em,
  start chain=going above,
  scale=0.5,
  every node/.style={scale=0.5}]
	 \node[bignode, gen_circle] (z) {$y_t$};
	 \node[bignode, gen_circle, left=1.5em of z, join] (u) {$u_t$};
	 \node[bignode, gen_circle, left=1.5em of u, join] (y) {$z_t$};
	 \node[bignode, gen_circle, below=0.8em of y, join] (x) {$x_t$};
	 \node[bignode, gen_circle, above=.8em of y, fill=black!15] (x1) {$x_{-t}$};
     \draw[->,thin] (x1.south) -> (y.north);
     \draw[->,thin] (x1.320) -> (u.120);
     \draw[->,thin] (x1.350) -> (z.130);
\end{tikzpicture}

==> graphical_plots/gumbel_2gaussian.tex <==
\begin{tikzpicture}
  [node distance=1.5em,
  start chain=going above,
  scale=0.5,
  every node/.style={scale=0.5}]
	 \node[bignode, gen_circle] (z) {$g_t$};
	 \node[bignode, gen_circle, below=0.8em of z, join] (u) {$u_t$};
	 \node[bignode, gen_circle, below=0.8em of u, join] (y) {$z_t$};
	 \node[bignode, gen_circle, below=0.8em of y, join] (x) {$x_t$};
\end{tikzpicture}

==> graphical_plots/gumbel_gaussian.tex <==
\begin{tikzpicture}
  [node distance=1.5em,
  start chain=going above,
  scale=0.5,
  every node/.style={scale=0.5}]
	 \node[bignode, gen_circle] (z) {$g_t$};
	 \node[bignode, gen_circle, below=0.8em of z, join] (y) {$z_t$};
	 \node[bignode, gen_circle, below=0.8em of y, join] (x) {$x_t$};
\end{tikzpicture}

==> graphical_plots/recurrent_gaussian.tex <==
\begin{tikzpicture}
  [node distance=1.5em,
  start chain=going above,
  scale=0.5,
  every node/.style={scale=0.5}]
	 \node[bignode, gen_circle] (z) {$z_t$};
	 \node[bignode, gen_circle, below=1.5em of z, join] (x) {$x_t$};
	 
     \draw[->,thin] (z.west)|-+(-3em,0)-> (z.west);
      \draw[->,thin] (z.east) -> (z.east)|-+(3em,0);
\end{tikzpicture}
